LOCOST: State-Space Models for Long Document Abstractive Summarization

State-space models are a low-complexity alternative to transformers for encoding long sequences and capturing long-term dependencies. We propose LOCOST: an encoder-decoder architecture based on state-space models for conditional text generation with long context inputs. With a computational complexity of $O(L \log L)$, this architecture can handle significantly longer sequences than state-of-the-art models that are based on sparse attention patterns. We evaluate our model on a series of long document abstractive summarization tasks. The model reaches a performance level that is 93-96% comparable to the top-performing sparse transformers of the same size while saving up to 50% memory during training and up to 87% during inference. Additionally, LOCOST effectively handles input texts exceeding 600K tokens at inference time, setting new state-of-the-art results on full-book summarization and opening new perspectives for long input processing.

==> emnlp2023-latex/6_conclusion.tex <==



==> emnlp2023-latex/related_work_florian.tex <==
\section{Related work}\label{sec:related-works}

\subsection{Long-inputs}
There are extensive work on NLP architectures for long texts. We will give some details about the most commons ones and the ones that are the most related to our work.

\paragraph{Efficient attention.} Based on the empirical observation that attention weights seems to be sparse, some models like \citet{bigbird} or \citet{longformer} propose to restrict the number of tokens to attend to in the computation of the attention weights. \citet{reformer} introduces a hash mechanism to select only the pertinent tokens for the attention computation.

\paragraph{Modified attention computation.} Some use modified computations of the attention weights. For example, \cite{linformer} aims at approximate the sequence's matrix $\mU \in \R^{L \times H}$ with random projections, which is justified by the Jonhson-Lindenstrauss lemma \cite{johnson-lindenstrauss}. It results of a matrix $\boldsymbol{\widetilde{U}} \in \R^{K \times H}$ with $K < L$, that can be interpreted as a sequence of $K$ artificial tokens and is therefore similar to our SSM-RATTN which compresses the input sequence into $r$ tokens. To the best of our knowledge this model has only been used for encoding tasks. More recently \citet{transformer-linear-time} proposed to use as well a linear approximation of attention, similar to the one of \citet{linformer}, with an extra full quadratic attention over a local window. Other models like \citet{transformer-xl} or \citet{compressive-transformer} try to save in memory previous tokens representation to enlarge the context window, without the full burden of attention.

\paragraph{Attention-free models.} Recently some models that doesn't use attention at all have been proposed. \citet{fnet} is a mixin model \citep{gmlp} that leverages DFT to encode efficiently a sequence in $\bigO(L \log L)$. This model matches the complexity of ours but it can only be used for encoding tasks, since the DFT is a non-causal mechanism. Another drawback of this mechanism is that the sequence length should be fixed, since the output of a DFT depends on the sequence length.

\paragraph{Global and local.} A lot of these mechanisms are found to be ineffective if used as is. They are therefore often used in conjunction of a local attention over a fixed length window. In other cases adding local attention simply improves performance.


\subsection{Long inputs summarization}
For long-inputs summarization the state of the arts models relies on extractive-abstractive models. They create a compressed representation of the input text with that can after be decoded using a classical transformer. We can mention \citet{seal} who propose to dynamically select the snippets based on what has already been decoded. \citet{dyle} propose to consider the extracted snippets as latent variables and adds a consistency loss between the extraction and the generation that helps to refine the snippets selection.

These models therefore does not encode the whole sequence, contrarily to previous approaches but according to the experiments in \citet{dyle}, they are the currently the best performing methods. We hope to propose a mechanism that is able to encode the whole sequence and to perform as well as these ones.

\subsection{Language models pretraining.}
Our work involved a large-scale pretraining. Several pretraining objectives have been proposed. For generation tasks, \citet{bart} proposed a denoising tasks as an unsupervised objective. Spans of text are masked out and should be retrieved by the model. Recent work in \citet{unilm} suggests that this objective is especially efficient. \citet{pegasus} proposed a similar objective but tailored to summarization by masking selected sentences, used as pseudo-summaries that minimizes the ROUGE-score \citep{rouge} with the rest of the text. PEGASUS model \citep{pegasus} was trained on both C4 and HugeNews dataset, with best performances attained on HugeNews. However, since this dataset has not been open-sourced, we conducted our experiments on the C4 dataset.

We noted that a lot of models were trained on a quite large amount of data. For example \citet{bart} and \citet{pegasus} were trained for 500 000k steps with a batch size of 8192. Due to resource limitations we followed the scale of the pretraining in \citet{t5}, which is smaller, but does not have the same objective than the other ones (not purely unsupervised).

\subsection{State-space models}

\paragraph{State-space models theory.} The theory of state-space models is presented in \citet{hippo}, and refined in \cite{s4d}. Despite the recursive formulation that is close to the one of RNN's, the authors derived some interesting guarantees around the approximation error and the gradient norm that are supposed to theoretically circumvent RNN's limitations. The fact that diagonal state-spaces are good approximations of dense state-spaces is exposed in \citet{s4d}.

\paragraph{First applicable models.} The first large-scale SSM models is S4 and has been proposed in \citet{s4d}. This model outperformed all the efficient transformers baselines on the Lng Range Arena benchmark \citep{efficient-transformers}, which motivated us to investigate this model. They applied it successfully for audio generation and encoding in \citet{sashimi}. However the S4 formulation was a bit limiting for text, due to the dependence of the formulation on the maximum input length. The first large-scale language modeling in \citet{gss} was therefore based on diagonal SSM (that builds upon \citet{dss}). They showed interesting properties like scaling and length generalization on code datasets. The models introduced later in \citet{s4d} proposed again a simplification of the computations we found well suited for text generation. Finally in \citet{train-hippo} give some advice on the initialization of SSM models that we followed.

==> emnlp2023-latex/tables/LRA_full.tex <==
\small
\begin{tabular}{l|cccccc|c|c}
\hline Dataset & Listops & Text & Retrieval & Image & Pathfinder & Path-X & Avg. \\
\hline Sequence length & $2 \mathrm{k}$ & $4 \mathrm{k}$ & $8 \mathrm{k}$ & $1 \mathrm{k}$ & $1 \mathrm{k}$ & $16 \mathrm{k}$ & - \\
\hline Random & 10.00 & 50.00 & 50.00 & 10.00 & 50.00 & 50.00 & 36.67 \\
Transformer (full) (Vaswani et al., 2017) & 36.37 & 64.27 & 57.46 & 42.44 & 71.40 & $\times$ & 53.66 \\
Transformer (window) & 15.82 & 52.98 & 53.39 & 41.46 & 66.63 & $\mathbf{x}$ & 46.71 \\
Sparse Trans. (Child et al., 2019) & 17.07 & 63.58 & 59.59 & 44.24 & 71.71 & $\mathbf{x}$ & 51.03 \\
Longformer (Beltagy et al., 2020) & 35.63 & 62.85 & 56.89 & 42.22 & 69.71 & $\mathbf{x}$ & 52.88 \\
Linformer (Wang et al., 2020b) & 35.70 & 53.94 & 52.27 & 38.56 & 76.34 & $\mathbf{x}$ & 51.14 \\
Reformer (Kitaev et al., 2020) & 37.27 & 56.10 & 53.40 & 38.07 & 68.50 & $\mathbf{x}$ & 50.56 \\
Sinkhorn Trans. (Tay et al., 2020) & 33.67 & 61.20 & 53.83 & 41.23 & 67.45 & $\mathbf{x}$ & 51.23 \\
Synthesizer (Tay et al., 2021a) & 36.99 & 61.68 & 54.67 & 41.61 & 69.45 & $\mathbf{x}$ & 52.40 \\
BigBird (Zaheer et al., 2020) & 36.05 & 64.02 & 59.29 & 40.83 & 74.87 & $\mathbf{x}$ & 54.17 \\
Linear Trans. (Katharopoulos et al., 2020) & 16.13 & 65.90 & 53.09 & 42.34 & 75.30 & $\mathbf{x}$ & 50.46 \\
Performer (Choromanski et al., 2021) & 18.01 & 65.40 & 53.82 & 42.77 & 77.05 & $\mathbf{x}$ & 51.18 \\
FNet (Lee-Thorp et al., 2022) & 35.33 & 65.11 & 59.61 & 38.67 & 77.80 & $\mathbf{x}$ & 54.42 \\
Nystromformer (Xiong et al., 2021) & 37.15 & 65.52 & 79.56 & 41.58 & 70.94 & $\mathbf{x}$ & 57.46 \\
Luna-256 (Ma et al., 2021) & 37.25 & 64.57 & 79.29 & 47.38 & 77.72 & $\mathbf{x}$ & 59.37 \\
FMMformer (Nguyen et al., 2021) & 36.74 & 67.84 & 81.88 & 45.10 & 72.12 & $\mathbf{x}$ & 60.74 \\
S4 (Gu et al., 2021) & 58.35 & 76.02 & 87.09 & 87.26 & 86.05 & 88.10 & 80.48 \\
MEGA-chunk (Ma et al., 2022) & 58.76 & 90.19 & 90.97 & 85.80 & 94.41 & 93.81 & 85.66 \\
SPADE (softmax-window) & 59.70 & 87.55 & 90.13 & $\mathbf{8 9 . 1 1}$ & $\mathbf{9 6 . 4 2}$ & 94.22 & 86.19 \\
SPADE (MEGA-chunk) & $\mathbf{6 0 . 5 0}$ & $\mathbf{9 0 . 6 9}$ & $\mathbf{9 1 . 1 7}$ & 88.22 & 96.23 & $\mathbf{9 7 . 6 0}$ & $\mathbf{8 7 . 4 0}$ \\
\hline LongS4D & $\mathbf{6 1 . 60}$ & x & x & x & x & x & x \\
\hline
\end{tabular}

==> emnlp2023-latex/tables/LRA_short.tex <==
\small
\begin{tabular}{l|cccccc|c}
\hline  & \textbf{Listops} & \textbf{Text} & \textbf{Retrieval} & \textbf{Image} & \textbf{Pathfinder} & \textbf{Path-X} & \textbf{Avg.} \\
\hline Sequence length & $2 \mathrm{k}$ & $4 \mathrm{k}$ & $8 \mathrm{k}$ & $1 \mathrm{k}$ & $1 \mathrm{k}$ & $16 \mathrm{k}$ & - \\
\hline Random & 10.00 & 50.00 & 50.00 & 10.00 & 50.00 & 50.00 & 36.67 \\
Transformer (full) \cite{attention_is_all_you_need} & 36.37 & 64.27 & 57.46 & 42.44 & 71.40 & \mbox{\ding{55}} & 53.66 \\

Longformer \cite{longformer} & 35.63 & 62.85 & 56.89 & 42.22 & 69.71 & \mbox{\ding{55}} & 52.88 \\

BigBird \cite{bigbird} & 36.05 & 64.02 & 59.29 & 40.83 & 74.87 & \mbox{\ding{55}} & 54.17 \\

FNet \cite{fnet} & 35.33 & 65.11 & 59.61 & 38.67 & 77.80 & \mbox{\ding{55}} & 54.42 \\

S4 \cite{s4} & 58.35 & 76.02 & 87.09 & 87.26 & 86.05 & 88.10 & 80.48 \\

MEGA-chunk \cite{mega} & 58.76 & 90.19 & 90.97 & 85.80 & 94.41 & 93.81 & 85.66 \\

SPADE (softmax-window, \citet{spade}) & 59.70 & 87.55 & 90.13 & $\mathbf{8 9 . 1 1}$ & $\mathbf{9 6 . 4 2}$ & 94.22 & 86.19 \\

SPADE (MEGA-chunk, \citet{spade}) & $6 0 . 5 0$ & $\mathbf{9 0 . 6 9}$ & $\mathbf{9 1 . 1 7}$ & 88.22 & 96.23 & $\mathbf{9 7 . 6 0}$ & $\mathbf{8 7 . 4 0}$ \\

\hline LongS4D (ours) & $\mathbf{6 1 . 60}$ & x & x & x & x & x & x \\
\hline
\end{tabular}

==> emnlp2023-latex/tables/SCROLLS_full.tex <==
\small
\begin{tabular}{l|ccccccccc|c}
\hline Model & Speed & NQA & QAS & QuAL & CNLI & SumS & QMS & GovR & Avg \\
\hline & F1 & F1 & EM & EM & $\mathbf{R}_{\mathrm{gm}}$ & $\mathbf{R}_{\mathrm{gm}}$ & $\mathbf{R}_{\mathrm{gm}}$ \\
\hline LongT5 (base) & 23.0 & 46.6 & 37.9 & 85.6 & 19.2 & 20.4 & 37.7 & 43.1 \\
CoLT5 (base) & 23.3 & 42.1 & 36.5 & 86.5 & 18.7 & 18.4 & 37.9 & 42.4 \\
LOCOST (base) & 14.6 & 25.6 & 25.0/27.1 & 78.4 & 33.4/8.1/19.7 & 29.2/7.1/19.1 & 56.5/26.8/28.9 & 30.31
%\hline LongT5-L & 45.3 & $0.3 / 3.0$ & 1.3 & 84.2 & 27.2 & 52.3 & 40.6 & 87.3 & 35.7 & 19.1 & 21.4 & 39.5 \\
%CoLT5-L & 45.3 & 5.0 & 2.0 & 84.5 & 27.7 & 49.8 & 39.9 & $\mathbf{8 8 . 7}$ & 35.9 & $\mathbf{2 0 . 5}$ & 21.0 & 39.7 \\
%\hline LONGT5-XL & 46.6 & $0.2 / 1.2$ & 0.4 & 85.3 & 29.3 & 53.1 & 46.0 & 88.2 & 35.9 & 19.4 & 21.3 & $\mathbf{4 0 . 5}$ \\
%CoLT5-XL & $\mathbf{4 7 . 4}$ & 2.3 & 0.5 & $\mathbf{8 6 . 1}$ & $\mathbf{3 1 . 1}$ & $\mathbf{5 3 . 9}$ & $\mathbf{4 8 . 1}$ & 88.4 & $\mathbf{3 6 . 1}$ & 20.0 & $\mathbf{2 2 . 5}$ & $\mathbf{4 0 . 5}$ \\
\hline
\end{tabular}

==> emnlp2023-latex/tables/arxiv.tex <==
\small
\begin{tabular}{lccc}
\hline & \multicolumn{3}{c}{ \textbf{arXiv} }\\
\textbf{Model} & R-1 & R-2 & R-L  \\
\hline Pegasus (base) & 34.81 & 10.16 & 22.50 \\
BigBird-RoBERTa (base) & 41.22 & 16.43 & 36.96 \\
LED
%\hline T5.1.1 (large - 1k input) & 39.79 & 14.02 & 36.23 \\
%T5.1.1 (large - 2k input) & 42.84 & 16.62 & 39.01 \\
%T5.1.1 (large - 4k input) & 44.51 & 18.20 & 40.62 \\
%T5.1.1 + PSG (large - 1k input) & 38.53 & 13.61 & 35.08 \\
%T5.1.1 + PSG (large - 2k input) & 42.85 & 16.50 & 38.99 \\
%T5.1.1 + PSG (large - 4k input) & 45.86 & 18.40 & 41.62 \\
LongT5 (base - 4k input) & 44.87 & 18.54 & 40.97 \\
\hline \name (base - 4k input) & 43.96 & 16.40 & 39.33 \\
\name (base - 8k input) & - & - & - \\

\hline
\end{tabular}

==> emnlp2023-latex/tables/booksum.tex <==
\tiny
\begin{tabular}{lccc|ccc|ccc|ccc}
\hline & \multicolumn{3}{c|}{ \textbf{arXiv} } & \multicolumn{3}{c|}{ \textbf{PubMed} } & \multicolumn{3}{c|}{ \textbf{Multi-News} } & \multicolumn{3}{c}{ \textbf{BookSum} } \\
\textbf{Model} & R-1/R-2/R-L & B & \% &  R-1/R-2/R-L & B & \% & R-1/R-2/R-L & B & \%  & R-1/R-2/R-L & B & \% \\
\hline Pegasus (base) & 34.81/10.16/22.5 & -- & 64.55  & 39.98/15.15/25.23 & -- & -- & 42.24/13.27/21.44 & -- & -- & -- & -- & --  \\
BigBird (base) & 41.22/16.43/36.96 & -- & 90.53 \\
LED & 17.26/2.57/15.7 & 56.12 & 46.27\\
%BART (base) + Unlimiformer & 56.6 & 26.3 & 27.6 & 34.7 & 8.5 & 19.9 & - & - & - \\
%PRIMERA + Unlimiformer & 57.4 & 26.2 & 28.0 &  33.3 & 7.6 & 18.9 & - & - & - \\
\hline
LongT5 & 45.18/18.36/40.98 & 69.37 & 100 & 47.94/22.50/44.19 & 59.96 & 100 & 46.22/18.14/42.53 & 61.12 & 100 & 35.78/7.24/33.74 & 46.68 & 100 \\
LOCOST (ours) & -- & -- & -- & 45.68/20.11/41.97 & 60.07 & 94.01 & 43.76/15.4/40.15 & 61.96 & 90.26 & 34.30/6.09/32.36 & 46.67 & 94.76\\
\hline
\end{tabular}

==> emnlp2023-latex/tables/length_generalization_arxiv.tex <==
\small
\begin{tabular}{l|ccc|ccc|c}
\hline & \multicolumn{3}{c|}{ \textbf{arXiv-4K} } & \multicolumn{3}{c|}{ \textbf{arXiv-8K} }  \\
\textbf{Model} & R-1 & R-2 & R-L & R-1 & R-2 & R-L & Gain (\%)  \\
\hline LongT5 & 45.18 & 18.36 & 40.98 & 45.76 & 19.06 & 41.6 & 1.81 \\
LOCOST & 43.82	& 16.96	& 39.66 & 44.65 & 17.77 & 40.48 &  2.45\\
%BART (base) + Unlimiformer & 56.6 & 26.3 & 27.6 & 34.7 & 8.5 & 19.9 & - & - & - \\
%PRIMERA + Unlimiformer & 57.4 & 26.2 & 28.0 &  33.3 & 7.6 & 18.9 & - & - & - \\
\hline
\end{tabular}

==> emnlp2023-latex/tables/pubmed.tex <==
\small
\begin{tabular}{lccc}
\hline & \multicolumn{3}{c}{ \textbf{PubMed} } \\
\textbf{Model} & R-1 & R-2 & R-L \\
\hline 
Transformer + PSG & 39.98 & 15.15 & 35.89 \\
BigBird-RoBERTa (base) & 43.70 & 19.32 & 39.99 \\
BigBird-PEGASUS (large) & 46.32 & 20.65 & 42.33 \\
%\hline T5.1.1 (large - 1k input) & 42.18 & 16.60 & 38.96 \\
%T5.1.1 (large - 2k input) & 45.51 & 19.55 & 42.10 \\
%T5.1.1 (large - 4k input) & 47.90 & 22.08 & 44.36 \\
%T5.1.1 + PSG (large - 1k input) & 43.34 & 17.55 & 40.10 \\
%T5.1.1 + PSG (large - 2k input) & 46.51 & 20.37 & 43.00 \\
%T5.1.1 + PSG (large - 4k input) & 48.94 & 22.92 & 45.4 \\
%LongT5 (large - 4k input) & 47.77 & 22.58 & 44.38 \\
LongT5 (base - 4k input) & 44.87 & 18.54 & 40.97 \\
\hline \name (base - 4k input) & - & - & - \\
\name (base - 8k input) & - & - & - \\
\hline
\end{tabular}

==> emnlp2023-latex/tables/summarization_datasets.tex <==
% \small
% \begin{tabular}{lcc|c|cc|c|cc|c}
% \hline & \multicolumn{3}{c}{ \textbf{arXiv} } & \multicolumn{3}{c}{ \textbf{PubMed} } & \multicolumn{3}{c}{ \textbf{Multi-News} } \\
% \textbf{Model} & R-1/R-2/R-L & B & \% &  R-1/R-2/R-L & B & \% & R-1/R-2/R-L & B & \%  \\
% \hline PEGASUS & 34.8/10.2/22.5 & -- & 64.55  & 40.0/15.2/25.2 & -- & -- & 42.2/13.3/21.4 & -- & --   \\
% BigBird & 41.2/16.4/37.0 & -- & 90.5 & -- & -- & -- & -- & -- & -- \\
% LED & 41.3/16.4/37.7 & 69.5 & 91.3 & -- & -- & -- & -- & -- & -- \\
% %BART (base) + Unlimiformer & 56.6 & 26.3 & 27.6 & 34.7 & 8.5 & 19.9 & - & - & - \\
% %PRIMERA + Unlimiformer & 57.4 & 26.2 & 28.0 &  33.3 & 7.6 & 18.9 & - & - & - \\
% \hline
% LongT5 & 45.18/18.36/40.98 & 69.37 & 100 & 47.94/22.50/44.19 & 59.96 & 100 & 46.22/18.14/42.53 & 61.12 & 100  \\
% LOCOST & 43.82/16.96/39.66 & 69.44 & 96.09 & 45.68/20.11/41.97 & 60.07 & 94.01 & 43.76/15.4/40.15 & 61.96 & 90.26 \\
% \hline
% \end{tabular}
